Accelerated Data-Flow Analysis

Acceleration in symbolic verification consists in computing the exact effect of some control-flow loops in order to speed up the iterative fix-point computation of reachable states. Even if no termination guarantee is provided in theory, successful results were obtained in practice by different tools implementing this framework. In this paper, the acceleration framework is extended to data-flow analysis. Compared to a classical widening/narrowing-based abstract interpretation, the loss of precision is controlled here by the choice of the abstract domain and does not depend on the way the abstract value is computed. Our approach is geared towards precision, but we don't loose efficiency on the way. Indeed, we provide a cubic-time acceleration-based algorithm for solving interval constraints with full multiplication.

==> OLD_JL_sec.flattening.tex <==
\newpage
\section{Flatenning}
\subsection{Graph associated to a constraint system}
As usual, constraint systems are represented by graphs. This representation provides three classes of constraint systems: \emph{acyclic}, \emph{flat} and \emph{sunny}.

A \emph{(labelled) graph} $G$ is a tuple $G=(N,\Sigma,\Delta)$ where $N$ is a set of \emph{nodes}, $\Sigma$ is a set of \emph{labels}, and $\Delta$ is a set of transitions $\Delta\subseteq N\times\Sigma\times N$. 
%
A \emph{path} in $G$ is an alternating sequence of nodes and labels denoted by $n_0\xrightarrow{a_1}n_1\cdots n_{k-1}\xrightarrow{a_k}n_k$ where $k\geq 0$ is the \emph{length} of the path, $n_0$, ..., $n_k$ are nodes in $N$ and $a_1$, ..., $a_k$ are labels in $\Sigma$ such that $(n_0,a_1,n_1)$, ..., $(n_{k-1},a_k,n_k)$ are in $\Delta$. The nodes $n_0$ and $n_k$ are respectivelly called the \emph{source} and the \emph{target} nodes. When these two nodes are equal to the same node $n$ and when the length of the path is greater than zero $k\geq 1$, the path is called a \emph{cycle} on $n$.
%
A \emph{strongly connected componant} of $G$ is an equivalence class for the equivalence relation $\equiv$ such that $n_1\equiv n_2$ if and only if there exists a path from $n_1$ to $n_2$ and a path from $n_2$ to $n_1$. A strongly connected componants $N'$ is said \emph{transient} if $\Delta\cap (N'\times \Sigma\times N')$ is empty.
%
A strongly connected componant $N'$ is said \emph{cylic} if there exists $k\geq 1$ \emph{distinct} nodes $n_0$, ..., $n_{k-1}$ and some labels $a_1$, ..., $a_k$ such that $\Delta\cap (N'\times \Sigma\times N')=\{(n_0,a_1,n_1),..., (n_{k-1},a_k,n_0)\}$.\\
%
A labelled graph $G$ is said \emph{acyclic} if there does not exist a cycle in $G$ (or equivalently any strongly connected componant is transient), and it is said \emph{flat} if its strongly connected componants are either transient or cyclic.\\

The \emph{graph $G=(\V\cup C, \Nat, \Delta)$ associated to a constraint system $C$} is defined by a set of nodes equal to the disjoint union of the set of variables $\V$ and the set of constraints $C$ and where $\Delta$ is the set of transitions $(X_i,i,c)$ and $(c,0,X)$ for each constraint $c\in C$ of the form $X\sqsupseteq f(X_1,\ldots,X_k)$.\\

A constraint system is said \emph{acyclic} or \emph{flat} if its associated graph is respectivelly \emph{acyclic} or \emph{flat}. Moreover, a non empty flat constraint system $C$ is said \emph{sunny} if $C$ is included into a cyclic strongly connected componant.


\begin{remark}
  In this paper, the nodes of the graphs associated to a constraint system are graphically represented either by a circle or a square following that they correspond to a variable or a constraint. See for instance the figure \ref{fig:exgraph}. 
\end{remark}

%%\begin{figure}
%%  \begin{center}
%%    \begin{picture}(60,24)(0,-12)
%%      \put(0,-12){\framebox(60,24){}}
%%      \node[NLangle=0.0,Nmr=0.0](n0)(8.0,0.0){$c_1$}
%%      \node[NLangle=0.0](n1)(28.0,0.0){$X$}
%%      \node[NLangle=0.0,Nmr=0.0](n2)(48.0,0.0){$c_2$}
%%      \drawedge(n0,n1){}
%%      \drawedge[curvedepth=8.0](n1,n2){$1$}
%%      \drawedge[curvedepth=-8.0](n1,n2){$2$}
%%      \drawedge(n2,n1){}
%%    \end{picture}
%%  \end{center}
%%  \caption{The labelled graph associated to $c_1:a\sqsubseteq X$ and $c_2:\textrm{add}(X,X)\sqsubseteq X$.\label{fig:exgraph}}
%%\end{figure}


\subsection{Unfolding of a set of constraints}
In the sequel $z$ denotes a function in $\V\rightarrow\V$ called a \emph{renaming function} of $\V$ and $(C,\rho_0)$ is an initialized constraint system.\\

Given a constraint $c'$ of the form $X'\sqsupseteq f(X_1',\ldots,X_n')$, we denote by $z(c')$ the constraint $z(X')\sqsupseteq f(z(X_1'),\ldots,z(X_n'))$ where the variables $X'$, $X_1'$, ..., $X_n'$ have been renamed thanks to renaming function $z$.\\

A constraint system $C'$ is called an \emph{unfolding} of $C$ by $z$ if the constraint $z(c')$ is either in $C$ or equal to a constraint of the form $X\sqsupseteq X$ for any constraint $c'\in C'$. 

\begin{figure}
  \begin{center}
    \begin{picture}(24,30)(-12,23)
      \put(-12,23){\framebox(24,30){}}
      %%\node[NLangle=0.0,Nmr=0.0](n0)(0.0,8.0){$c_1$}
      \node[NLangle=0.0](n1)(0,28.0){$X$}
      \node[NLangle=0.0,Nmr=0.0](n2)(0,48.0){$c$}
      %%\drawedge(n0,n1){}
      \drawedge[curvedepth=8.0](n1,n2){$1$}
      \drawedge[curvedepth=-8.0,ELside=r](n1,n2){$2$}
      \drawedge(n2,n1){}
    \end{picture}
  \begin{picture}(48,30)(-24,23)
      \put(-24,23){\framebox(48,30){}}
      %%\node[NLangle=0.0,Nmr=0.0](n0)(-12.0,8.0){$c_3$}
      %%\node[NLangle=0.0,Nmr=0.0](n0p)(12.0,8.0){$c_4$}
      \node[NLangle=0.0](n1)(-12,28.0){$X$}
      \node[NLangle=0.0](n1p)(12,28.0){$X'$}
      \node[NLangle=0.0,Nmr=0.0](n2)(0,48.0){$c'$}
      %%\drawedge(n0,n1){}
      %%\drawedge(n0p,n1p){}
      \drawedge[curvedepth=8.0](n1,n2){$1$}
      \drawedge[curvedepth=-8.0,ELside=r](n1p,n2){$2$}
      \drawedge(n2,n1){}
    \end{picture}
    \end{center}
  \caption{The graphs associated to the contraint systems $C=\{c\}$ and $C'=\{c'\}$ where $c$ and $c'$ are respectivelly the constraints $X\sqsupseteq \textrm{add}(X,X)$ and $X\sqsupseteq \textrm{add}(X,X')$.\label{fig:exgraph}}
\end{figure}

\begin{example}
   Let us consider the contraint systems $C=\{c\}$ and $C'=\{c'\}$ represented in figure \ref{fig:exgraph} where $c$ and $c'$ are respectivelly the constraints $X\sqsupseteq \textrm{add}(X,X)$ and $X\sqsupseteq \textrm{add}(X,X')$. Note that $C'$ is an unfolding of $C$ by the renaming $z$ defined by $z(X)=X=z(X')$.
\end{example}

Consider an unfolding $C'$ of $C$ by the renaming function $z$ and observe that $\least_{C}\circ z$ is a solution of $C'$. Thus by minimality of $\least_{C'}$, we get $\least_{C'}\sqsubseteq\least_{C}\circ z$ and we have proved the following relation:
$$\least_{C'}\circ z^{-1}\sqsubseteq \least_C$$
where the valuation $\rho'\circ z^{-1}$ is defined, with slightly abusing notation, for any valuation $\rho'$ and for any $X\in\V$ by 
$$\rho'\circ z^{-1}(X)=\bigsqcup_{X'\in z^{-1}(X)}\rho'(X')$$
When the relation $\least_{C'}\circ z^{-1}\sqsubseteq\textrm{least}_C$ is in fact an equality, the unfolding $C'$ is said \emph{complete}.




\subsection{Flatenning}
In this section we introduce the flatenning framework for computing the least solution of some constraint systems.\\


This framework is based on the fact that there exists complete unfolding of some constraint systems such that the associated graph has a special structure. For instance, the following proposition illustrate this idea on constaint systems $C$ whose the least solution is a \emph{finite propagation}. We say that $\least_C$ is \emph{finite propagation} if there exists a sequence $c_1, \ldots, c_k$ of constraints in $C$ such that $\least_C = (\one \sqcup c_k) \circ \cdots \circ (\one \sqcup c_1)(\bot)$.
\begin{proposition}\label{prop:ac}
  The least solution of a constraint system $C$ is a finite propagation if and only if there exists a complete acyclic unfolding of $C$.
\end{proposition}
\begin{proof}
   First assume that $\least_C$ is a finite propagation. Thus there exists $k\geq 0$ constraints $c_1$, ..., $c_k$ in $C$ such that $\least_C$ is equal to $(\one\sqcup c_k)\circ\cdots\circ (\one\sqcup c_1)(\bot)$. The constraint $c_i$ is denoted by $X_i\sqsupseteq f_i(X_{i,1},\ldots, X_{i,n_i})$. Let $\X$ be the finite set of variables appearing in $c_1$, ..., $c_k$. Since $\V$ is infinite whereas $\X$ is finite, we can denote by $(X,i)\in \X\times\finiteset{0}{k}$ some distinct variables in $\V\moins \X$. Let us consider the constraint system $C'$ containing the constraint $c'_{X,i}$ indexed by $X\in\X$ and $1\leq i\leq k$, and equals to:
   $$
   \begin{cases}
   (X,i)\sqsupseteq (X,i-1) & \text{if }X\not=X_i\\
   (X,i)\sqsupseteq f_i((X_{i,1},i-1),\ldots,(X_{i,n_i},i-1)) & \text{if }X=X_i\\
   \end{cases}
   $$
   Let $z$ be the renaming function defined by $z((X,i))=X$ if $X\in\X$ and $0\leq i\leq k$ and that lets unchanged the other variables. Just observe that $C'$ is a complete unfolding of $C$ by $z$ and the graph associated to $C'$ is acyclic.
   
   Converselly, assume that there exists a complete acyclic unfolding $C'$ of $C$ by a renaming function $z$. Since the graph $G'$ associated to $C'$ is acyclic, the constraints in $C'$ can be ordered into $c'_1$, ..., $c'_k$ such that if there exists a path in $G'$ from $c'_i$ to $c'_j$ then $i\leq j$. Observe that $\least_C$ is equal to $(\one\sqcup z(c'_1))\circ\cdots\circ (\one\sqcup z(c'_r))(\bot)$. By removing in the previous composition the functions $(\one\sqcup z(c'_i))$ if $z(c'_i)$ is a constraint of the form $X\sqsupseteq X$, we have proved that there exists some constraints $c_1$, ..., $c_k$ in $C$ such that $\least_C$ is equal to $(\one\sqcup c_1)\circ\cdots\circ (\one\sqcup c_k)(\bot)$. Thus $\least_C$ is a finite propagation. 
   \qed	  
\end{proof}

Naturally, there exists constraint systems $C$ whose the least solution is not a finite propagation. The previous proposition shows that the graph associated to any complete unfolding of $C$ always contains a cycle. In order to get the least solution of such a constraint system we consider the class of \emph{constraint systems} that has a complete unfolding.\\


\begin{definition}
  A \emph{flattening} of a constraint system is a flat unfolding. A constraint system is said \emph{flattable} if it has a complete flattening.
\end{definition}

Naturally, by definition, if the least solution of a constraint system $C$ is a finite propagation, then the 

from a sequence $c_1$, ..., $c_k$ of constraints such that $\least_C$ is equal to $(\one\sqcup c_k)\circ\cdots\circ (\one\sqcup c_1)(\bot)$ we can naturally extract a complete flattening of $C$ (see for instance the proof of proposition \ref{prop:ac}). This technique can be extended to the flattable constraint system thanks  \emph{sunny} constraint system.\\

A non-empty constraint system $C$ is said \emph{sunny} 





 

 propagating one by one the contraints we deduce the least solution. Moreover, a complete flattening can be extracted from this propagation (see for instance the proof of proposition \ref{prop:ac}). In the remaining of this section, this approach is extended to any flattable set of constraints.


Such a computation seems more natural than computing an unfolding with an acyclic associated graph and then check if this unfolding is complete. In order to extend these technique for flattable constraint systems, 

That means that a complete unfolding with an acyclic associated graph can be obtained by such a method.



Let us consider the graph $G$ associated to a flat set of constraints and a strongly connected componant of $G$ containing at least one contraint. 

let $C'$ be the set of constraints in a strongly connected componant of $G$. Observe that $C'$ may be empty or the graph associated to $C'$ may be not cyclic (see for instance example \ref{ex:sunny}). 





\begin{example}\label{ex:sunny}
  Let us consider the sunny constraint system $C=\{c\}$ where $c$ is the constraint $X\sqsupseteq \textrm{add}(X,Y)$. The graph associated to $G$ has two strongly connected componants $N_1=\{X,c\}$ and $N_2=\{Y\}$.
\end{example}
 

observe that for any strongly connected componant 

 and let $G$ be the graph associated 




A valuation $\rho$ is said \emph{computable by flattening} if there exists a flattening $(C',z)$ of $C$ such that $\rho=\textrm{least}_{C'}\circ z^{-1}$. Note that a valuation computable by propagation is also computable by a flattening $(C',z)$ such that the graph $G_{C'}$ is \emph{acyclic}. Observe that if $\textrm{prop}_c(\rho)\sqsubseteq\rho$ for any $c\in C$ then $\rho=\textrm{least}_{C}$ and the least solution of $C$ is computable by flattening. In such a case, the flattening is said \emph{complete} and the set of constraints $C$ is said \emph{flattable}. 









%%A labelled graph $G$ is said \emph{sunny} if there exists $k\geq 1$ \emph{distinct} nodes $n_0$, ..., $n_{k-1}$ and some labels $l_1$, ..., $l_k$ such that $\Delta$ is included in $\{(n_0,l_1,n_1),..., (n_{k-1},l_k,n_0)\}\cup ((N\moins N_0)\times L\times N_0)$ where $N_0$ is the set of nodes $n_0$, ..., $n_{k-1}$. Observe that any cylic graph is sunny but the converse is not true. This unusual clas of graphs will be intensivelly used in the sequel.






%%\begin{example}
%%  The labelled graph associated to the constraints $c_1:a\sqsubseteq X$ and $c_2:f(X,X)\sqsubseteq X$ is represented in figure \ref{fig:exgraph}.
%%\end{example}








\newpage

- graph associated with a constraint system (or in the previous section ?)

- notion of sunny graph   or   cyclic graph + $\rho_0$

- flatenning

- generic algorithm and theorem on termination


==> OLD_sec.convexconstraints.tex <==
- definition of convex constraints (f : AX <= B |-> X := X + C)

- computation of the least fixpoint for a single loop (i.e. for a single constraint and an initial valuation)

- examples showing that [Gonnord] does not compute the least fix-point (with their method,  iteration does not terminate when $P_0$ is not included in the guard), and does not compute the convex hull of the concrete least fixpoint.

- even for a sunny with polyhedral guards only (no trasnslation), the least fixpoint is not a polyhedron with rational coefficients.

